Finite-state Strategies in Delay Games (full version)

What is a finite-state strategy in a delay game? We answer this surprisingly non-trivial question by presenting a very general framework that allows to remove delay: finite-state strategies exist for all winning conditions where the resulting delay-free game admits a finite-state strategy. The framework is applicable to games whose winning condition is recognized by an automaton with an acceptance condition that satisfies a certain aggregation property. Our framework also yields upper bounds on the complexity of determining the winner of such delay games and upper bounds on the necessary lookahead to win the game. In particular, we cover all previous results of that kind as special cases of our uniform approach.

==> content/automatatrans.tex <==

Let $\aut = (Q \times M, \SigmaI\times \SigmaO, q_\initmark, \delta, \acc)$ and $\mon = (M, \init, \update)$ be given.

We define $\autb = (Q, \R \times Q, (q_\initmark,m_\initmark), \delta' \acc')$ with
\begin{itemize}
	\item some arbitrary~$m_\initmark \in M$,
	\item $\delta'((q,m),(S,q')) = $, and
	\item $(q_0, m_0) (q_0, m_0) (q_0, m_0) \cdots \in \acc'$ if, and only if, 
\end{itemize}


==> content/explicit.tex <==



==> content/implicit.tex <==
\todo{rename section to succinct?}





% ---
% Represent transition function and output function as transducers. We need to figure out what information these transducers need upfront (e.g., the state that should be reached). 
% 
% Results
% \begin{itemize}
% 	\item Upper bound of $2^{nd}$ on the number of states for the output function transducer: remember one completion taking automaton to each state reachable by currently processed word\todo{what about upper bound for transition transducer?}
% 	\begin{theorem}
% 		Martin 
% 	\end{theorem}
% 	\item Matching $2^{nd}$ lower bound: combine $2^n$ lower bound on necessary lookahead with copying. 
% 	\begin{theorem}
% 		Sarah
% 	\end{theorem}
% \item The transducer in transducer approach is \myquot{better} than explicit approach for identity winning condition
% 
% 
% 	\item The approach is not better for the block-reversal condition. 
% \begin{example}
% 	Sarah (where is the difference to thm 4?)
% \end{example}
% 	\item But it cannot be strictly worse than lookup-table approach, as we can implement on-the-fly evaluation in transducer.  
% \begin{theorem}
% 		Martin
% \end{theorem}
% \end{itemize}
% ---


